Ecovisor: A Virtual Energy System for Carbon-Efficient Applications

Cloud platforms' rapid growth is raising significant concerns about their carbon emissions. To reduce emissions, future cloud platforms will need to increase their reliance on renewable energy sources, such as solar and wind, which have zero emissions but are highly unreliable. Unfortunately, today's energy systems effectively mask this unreliability in hardware, which prevents applications from optimizing their carbon-efficiency, or work done per kilogram of carbon emitted. To address this problem, we design an "ecovisor", which virtualizes the energy system and exposes software-defined control of it to applications. An ecovisor enables each application to handle clean energy's unreliability in software based on its own specific requirements. We implement a small-scale ecovisor prototype that virtualizes a physical energy system to enable software-based application-level i) visibility into variable grid carbon-intensity and renewable generation and ii) control of server power usage and battery charging/discharging. We evaluate the ecovisor approach by showing how multiple applications can concurrently exercise their virtual energy system in different ways to better optimize carbon-efficiency based on their specific requirements compared to a general system-wide policy.

==> evaluation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/ml_training_application/ml_train_effdet_d1_coco.pdf}
%\vspace{-0.1cm}
\caption{\emph{Carbon emissions and runtime for distributed ML training using different carbon reduction policies.}}
%\vspace{-0.2cm}
\label{fig:reducing-carbon}
\end{figure}

% \begin{figure*}[t]
% \centering
% \begin{tabular}{@{}c@{}c@{}c@{}}
% \includegraphics[width=0.32\linewidth]{figures/blast/carbon_rate_emissions.pdf} &
% \includegraphics[width=0.32\linewidth]{figures/blast/resources.pdf} &
% \includegraphics[width=0.32\linewidth]{figures/blast/runtime_emissions_bargraph.pdf} \\
% %\vspace{-0.2cm}
% % (a) Carbon Rate and Emissions  & (b) Resource Usage and Carbon-intensity & (c) Runtime and Carbon Emissions
% (a) & (b) & (c) 
% \end{tabular}
% \caption{\emph{Carbon rate and carbon emissions (a) and resource usage and carbon intensity (b) over time for a representative BLAST job under different carbon rate-limiting policies.  Total running time and carbon emissions for the same experiment.}}
% \label{fig:rate-limiting}
% %\vspace{-0.3cm}
% \end{figure*}

\begin{figure}[t]
    \centering
    \begin{tabular}{c}
    \includegraphics[width=\columnwidth]{figures/blast/carbon_rate_emissions.pdf}\\
    (a) Carbon Rate and Emissions\\
    \includegraphics[width=\columnwidth]{figures/blast/resources.pdf}\\
    (b) Resource Usage and Carbon-intensity\\
    \includegraphics[width=\columnwidth]{figures/blast/runtime_emissions_bargraph.pdf}\\
    (c) Runtime and Carbon Emissions\\
    \end{tabular}
    %\vspace{-0.2cm}
    \caption{\emph{Carbon rate and carbon emissions (a) and resource usage and carbon intensity (b) over time for a representative BLAST job under different carbon rate-limiting policies.  Total running time and carbon emissions for the same experiment (c).}}
    %\vspace{-0.2cm}
    \label{fig:rate-limiting}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{tabular}{c}
%     \includegraphics[width=0.4\textwidth]{figures/blast/carbon_rate_emissions.pdf}\\
%     (a) Carbon rate and emissions\\
%     \includegraphics[width=0.4\textwidth]{figures/blast/resources.pdf}\\
%     (b) Resource usage and carbon intensity\\
%     \includegraphics[width=0.4\textwidth]{figures/blast/runtime_emissions_bargraph.pdf}\\
%     (c) Rate-limiting policies\\
%     \end{tabular}
%     \vspace{-0.15cm}
%     \caption{\emph{Carbon rate and carbon emissions (a) and resource usage and carbon intensity (b) over time for a representative BLAST job under different carbon rate-limiting policies.  Total running time and carbon emissions for the same experiment.}}
%     \vspace{-0.2cm}
%     \label{fig:rate-limiting}
% \end{figure}

%These applications include different types of data-parallel batch applications, as well as an interactive web application.   

The purpose of our evaluation is to highlight the rich policy space defined by our ecovisor's narrow API.  Specifically, we show how our ecovisor can support a variety of carbon-efficiency optimizations for different types of applications.  Importantly, these applications can operate concurrently on the same infrastructure.  In some cases, we re-implement and improve upon applications from prior work implemented on dedicated platforms~\cite{wait-awhile}.  Of course, our evaluation does not cover all possible uses of an ecovisor, as we expect there are numerous potential carbon-efficiency optimizations and simplifying abstractions for different types of applications that have yet to be developed.  A key goal of our system (as with any system) is to enable the development of these new optimizations and abstractions, while also supporting existing work.






%We evaluate our ecovisor by showing how it can support carbon-efficiency optimizations across many applications.  
%As mentioned in \Section\ref{sec:introduction}, while optimizing energy-efficiency has been well-studied in prior work, there is much less work on optimizing carbon-efficiency.  An important goal of an ecovisor is to enable carbon-efficiency optimizations.

\subsection{Reducing Carbon}
\label{sec:reducing}

% XXX What was the carbon threshold for WaitAWhile?  30th percentile for 48-hour windows chosen. Epoch is a pass over the training data.  The origin paper of EfficientDet-d1 model reports that they train the model for 300 epochs (and also take days or weeks for one run). We use batch size of 8 per GPU, which is the largest possible for Tesla V100 GPU. For other parameters, we follow the setting of origin paper[1]: Preprocessing: horizontal flipping and scale jittering, SGD Optimizer with momentum 0.9 and weight decay 4e-5, Batch norm decay 0.99 and epsilon 1e-3. Need to say something about GPUs here and in the implementation section. 

A basic approach to optimizing carbon-efficiency is to simply halt execution when grid power's carbon-intensity increases beyond some threshold.  Recent work, called WaitAWhile, quantifies the tradeoff between carbon emissions and job completion time using this approach~\cite{wait-awhile}.  We apply the same approach using our ecovisor to training a distributed ML model using grid power.  Specifically, we train the EfficientDet-d1 object detection model~\cite{efficientdet} on the Microsoft COCO dataset~\cite{coco} for one epoch using pytorch.  The model training job runs on grid power with a variable carbon footprint, which we simulate based on data from the carbon emissions of the California Independent System Operation (CAISO)~\cite{caiso} in 2020.  Since carbon emissions vary, we ran the experiment ten times and randomly selected the job arrival each time.  We set the carbon threshold based on the 30$^{th}$\% of carbon-intensity in each run.  We compared the WaitAWhile policy with a carbon-agnostic policy that simply runs the job, and a new Wait\&Scale policy we developed, which is the same as WaitAWhile but also scales up resource (and energy) usage when carbon emissions are low.  Our WaitAWhile and carbon-agnostic policies run the job on 4 GPUs by default, while our Wait\&Scale (2$\times$) policy simply scales up to 8 GPUs when below the carbon threshold, and our Wait\&Scale (3$\times$) scales up to 12 GPUs. 

Figure~\ref{fig:reducing-carbon} shows the results, where the error bars represent the standard deviation across the ten experiments.  As expected, the carbon-agnostic policy finishes in the shortest time but incurs the highest carbon emissions, while the WaitAWhile policy reduces carbon emissions by an average of $22.3$\%, but increases the running time by $9.7$$\times$.  The WaitAWhile policy also exhibits a highly volatile job runtime, since jobs that happen to start executing during a long high-carbon period are forced to stop and wait until the carbon-intensity decreases. Wait\&Scale (2$\times$) achieves a similar carbon reduction of $19.2$\%  but with a significantly lower runtime penalty (of $2.3$$\times$).   Unfortunately, scaling up offers diminishing carbon reductions as Wait\&Scale (3$\times$) only reduces carbon emissions by $5.82$\% with a similar runtime penalty as Wait\&Scale (2$\times$) (of $2.1$$\times$).  In this case, scaling up requires more coordination among nodes, which causes synchronization delays that limit speed-up and decrease energy-efficiency.  This experiment shows that these characteristics also affect carbon-efficiency.  Since synchronization delays differ across applications, the scale factor that optimizes carbon-efficiency will vary across applications, and may also change with the carbon-intensity. Finally, both Wait\&Scale policies exhibit less volatility in job runtimes compared to WaitAWhile because they are more aggressive about exploiting low-carbon periods when they are available to get work done. 

\subsection{Rate-limiting Carbon}
%% XXX From Abel: Yes, it is embarrassingly parallel and scales efficiently. There is a limit set by the DNA input (I used BLAST Input 235), from where after scaling beyond ~30 cores, the central queue task server has to more tasks to serve and it just wait for results and the extra nodes become mostly idle. If I increase the DNA input, this may be hidden, but the overall runtime for each experiment will also increase. I have inputs 480 [~0.5h] and 1080 [~1h], though I am not sure we need that.

A disadvantage of the simple carbon reduction policies above is that applications cannot make any forward progress during high carbon periods.  To address this problem, applications can use our ecovisor to rate-limit or cap their carbon emissions  at a specified amount over time.  Rate-limiting carbon enables applications to always make forward progress, albeit less during periods of high carbon-intensity. Of course, given such a carbon cap, grid power's variable carbon-intensity dictates a variable amount of grid power available to applications.   Applications can use the COP and ecovisor API to adjust their power usage and carbon emissions using horizontal and vertical scaling.   We demonstrate a policy for rate-limiting carbon using BLAST (Basic Local Alignment Search Tool), which is a commonly-used parallel application that searches for similarities in nucleotide or protein sequences~\cite{blast}.  We use a version of BLAST that is elastic, and thus can horizontally scale the number of containers it uses at runtime~\cite{tigres}. 

Figure~\ref{fig:rate-limiting} shows the results by comparing the carbon emissions and running time from executing BLAST under a carbon-agnostic policy that does not vary resource usage with carbon-intensity, and dynamic policies that vary resource and power usage as carbon-intensity varies to adhere to a specified rate of carbon emissions.  We implement two dynamic policies: one that only uses horizontal scaling to adjust power usage, and one that uses both horizontal and vertical scaling.  We also show the pseudo-code for the horizontal auto-scaler using our ecovisor API in Algorithm 1. Figure~\ref{fig:rate-limiting}(a) shows a time-series of carbon emissions for each policy, as well as the specified carbon rate (in this case, 37mg$\cdot$CO$_2$/W), while Figure~\ref{fig:rate-limiting}(b) shows the number of nodes allocated by each policy, as well as the grid's carbon-intensity.  As expected, our dynamic policies increase (and decrease) resource and energy usage when carbon-intensity decreases (and increases).  Our dynamic policy that combines both horizontal and vertical scaling is able to better match the specified carbon rate because it provides more fine-grained control of each node's power usage.  For carbon-intensity, we use a representative 48 hour period from the CAISO trace above. 

%\vspace{-0.3cm}
\begin{algorithm}[t]
{\scriptsize
\caption{Horizontal Auto-Scaler Policy}
\label{alg.horiz}
\begin{algorithmic}[1]
\REQUIRE \ target\_carbon\_rate\\
\FOR{each t$=1,2, \dots$}
\STATE $app\_power =$ {\fontfamily{qcr}\selectfont get\_app\_power()}\\
\STATE $grid\_carbon = $ {\fontfamily{qcr}\selectfont get\_grid\_carbon()}\\
\STATE $app\_carbon = app\_power \times grid\_carbon$\\
\STATE $delta\_carbon = app\_carbon - target\_carbon\_rate$\\
%\STATE $delta\_containers = int(delta\_carbon/$\\
%\STATE $ \quad \quad \quad \quad \quad \quad \quad \quad $ {\fontfamily{qcr} \selectfont get\_container\_carbon())}\\
\STATE ${delta\_containers = \Bigl \lfloor \dfrac{delta\_carbon}{\fontfamily{qcr} \selectfont get\_container\_carbon()}\Bigr\rfloor}$
\STATE $containers(t) = containers(t-1) + delta\_containers$\\
% \STATE $CO2_{trend} = \nabla CO2_{intensity}(t)$ %{\fontfamily{qcr}\selectfont \textbf{\#}Gradient of CO2(t)}
% \STATE $CO2_{overhead} = app_{energy}(t)*CO2_{trend}$
% \STATE $rsrc_{alloc} = \lfloor\frac{|CO2(t) - CO2_{target}|}{CO2_{overhead}}\rfloor$
%\STATE \textbf{return} $rsrc_{alloc}$
\ENDFOR
\end{algorithmic}
}
\end{algorithm}
% \vspace{-0.4cm}
%=======
%
%Algorithm \ref{alg.horiz} calculates a delta (line 5) to the  of the CO2 intensity function at point $t$ to calculate its slope and estimate the CO2 overhead/savings when adding ($\nabla > 0$) and removing resources ($\nabla < 0$) to/from the application. When $\nabla \sim 0$, we do not change the allocation.
%Figure~\ref{fig:rate-limiting} shows the results by comparing the carbon emissions and running time from executing BLAST under a carbon-agnostic policy that does not vary resource usage with carbon intensity, and dynamic policies that vary resource and power usage as carbon intensity varies to adhere to a specified rate of carbon emissions.  We implement two dynamic policies, both which are described by Algorithm \ref{alg.horiz}: one that only uses horizontal scaling to adjust power usage, and one that uses both horizontal and vertical scaling.  Figure~\ref{fig:rate-limiting}(a) shows a time-series of carbon emissions for each policy, as well as the specified carbon rate (in this case, 37mg$\cdot$CO$_2$/W), while Figure~\ref{fig:rate-limiting}(b) shows the number of nodes allocated by each policy, as well as the grid's carbon intensity.  As expected, our dynamic policies increase (and decrease) resource and energy usage when carbon intensity decreases (and increases).  Our dynamic policy that combines both horizontal and vertical scaling is able to better match the specified carbon rate because it provides more fine-grained control of each node's power usage.  For carbon-intensity, we use a representative 48 hour period from the CAISO trace above. 
%>>>>>>> ecd2112c61ead5004a9ed11ab4eed0840d344d48
%=======
%Algorithm \ref{alg.horiz} calculates a delta (line 5) to the target carbon rate to estimate how many resources can be added ($delta\_carbon > 0$) and removed ($delta\_carbon < 0$) from the application. When $delta\_carbon \sim 0$, no changes in the allocation is made.
%Figure~\ref{fig:rate-limiting} shows the results by comparing the carbon emissions and running time from executing BLAST under a carbon-agnostic policy that does not vary resource usage with carbon intensity, and dynamic policies that vary resource and power usage as carbon intensity varies to adhere to a specified rate of carbon emissions.  We implement two dynamic policies, both which are described by Algorithm \ref{alg.horiz}: one that only uses horizontal scaling to adjust power usage, and one that uses both horizontal and vertical scaling.  Figure~\ref{fig:rate-limiting}(a) shows a time-series of carbon emissions for each policy, as well as the specified carbon rate (in this case, 37mg$\cdot$CO$_2$/W), while Figure~\ref{fig:rate-limiting}(b) shows the number of nodes allocated by each policy, as well as the grid's carbon intensity.  As expected, our dynamic policies increase (and decrease) resource and energy usage when carbon intensity decreases (and increases).  Our dynamic policy that combines both horizontal and vertical scaling is able to better match the specified carbon rate because it provides more fine-grained control of each node's power usage.  For carbon-intensity, we use a representative 48 hour period from the CAISO trace above. 
%>>>>>>> 63c4e3ef1d1008e253f96c3cd58d3b2252d1dfd2

Finally, Figure~\ref{fig:rate-limiting}(c) shows that our dynamic rate-limiting policies reduce carbon emissions compared to the static policy without increasing running time, and thus improve carbon-efficiency.   In particular, using only horizontal scaling reduces carbon emissions by 19\%, while using horizontal and vertical scaling reduces it by 27\%.  Note that, unlike EfficientDet-d1, BLAST is close to embarrassingly parallel, and thus scales up much more efficiently to match the specified carbon rate when carbon intensity decreases.  Parallel applications with data synchronizations, such as EfficientDet-d1 above, would perform poorly under these policies, since blindly scaling up during periods of low carbon to match a specified carbon rate would be highly inefficient. 



\subsection{Budgeting Carbon}

While the policies above are effective at reducing and regulating carbon emissions for delay-tolerant batch applications, they are not appropriate for interactive applications, since periods of high carbon-intensity may not provide enough energy to satisfy the workload.   In this case, enforcing a carbon budget over a longer time period, e.g., a week or month, rather than a carbon rate is more appropriate.   Carbon budgets can provide interactive applications useful flexibility to increase their carbon emissions to satisfy load when it is high, and then effectively pay these carbon emissions back when load is low.  Carbon budgeting serves a similar purpose as storing energy in batteries when carbon emissions are low, and then using it when carbon emissions are high.  However, energy storage capacity is expensive, and thus can only time-shift low-carbon energy over relatively short periods, e.g., a day, while carbon budgets can operate over arbitrarily long periods, e.g., weeks, months, or years. Of course, the SLOs an interactive application can provide, e.g., on latency and throughput, are a function of its carbon budget, grid carbon intensity, and workload, which dictates its server load and power usage. 

\begin{figure}[t]
    \centering
    \begin{tabular}{c}
    %\includegraphics[width=0.4\textwidth]{./figures/webserver_application/webapp_setup.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/webserver_application/webapp_setup.pdf}\\
    (a) Carbon intensity and workload\\
    %\includegraphics[width=0.4\textwidth]{./figures/webserver_application/webapp_results.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/webserver_application/webapp_results.pdf}\\
    (b) 95p latency\\
    %\includegraphics[width=0.4\textwidth]{./figures/webserver_application/webapp_carbon.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/webserver_application/webapp_carbon.pdf}\\
    (c) Carbon rate\\
    %\includegraphics[width=0.4\textwidth]{./figures/webserver_application/webapp_workers.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/webserver_application/webapp_workers.pdf}\\
    (d) Workers\\
    \end{tabular}
    %\vspace{-0.2cm}
    \caption{\emph{Comparing a carbon rate-limiting and carbon budgeting policies for a distributed web server.}}
    %\vspace{-0.2cm}
    \label{fig:webserver-app}
\end{figure}

% XXX Need a few more details on distributed web application here, e.g., Wikipedia trace, size of cluster, etc.
Our ecovisor enables platforms to enforce carbon budgets and applications to respond to them. To illustrate the benefits of carbon budgeting, we deploy a distributed web application using our ecovisor prototype. The application includes a front-end load balancer that distributes web requests across a cluster, and serves a copy of Wikipedia.  The application uses horizontal scaling to regulate power usage by adding and removing containers from the load balancer's set of active servers.  We subject the application to variable workload demand based on a real-world trace covering 48 hours, and record the latency to satisfy requests~\cite{wikipedia-trace}.  We then run the application when rate-limiting carbon to 20 mg$\cdot$CO$_2$/W, and also under a carbon budget that is equivalent to the product of the same rate and the length of the trace.  In the carbon budgeting case, we horizontally scale the containers up and down to enforce an SLO on the 95$^{th}$\% latency of 50ms.   

\begin{figure}[t]
    \centering
    \begin{tabular}{c}
    %\includegraphics[width=0.4\textwidth]{./figures/spark/solar_trace.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/spark/solar_trace.pdf}\\
    (a) Solar power output\\
    %\includegraphics[width=0.4\textwidth]{./figures/spark/worker_plot_0.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/spark/worker_plot_0.pdf}\\
    (b) Worker trend with no battery\\
    %\includegraphics[width=0.4\textwidth]{./figures/spark/worker_plot_60.pdf}\\
    \includegraphics[width=\columnwidth]{./figures/spark/worker_plot_60.pdf}\\
    (c) Worker trend with 600Wh battery\\
    \end{tabular}
    %\vspace{-0.1cm}
    \caption{\emph{Number of workers with (c) and without (b) a battery when running a Spark job on the solar in (a).}} 
%    Number of active workers (right y-axis) for a Spark application running on solar power (left y-axis) over time (x-axis) using different battery capacities (top).  Total running time (left y-axis) and solar energy usage (right y-axis) as a function of battery capacity (x-axis) for the same application.}}
    %\vspace{-0.2cm}
    \label{fig:spark}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/spark/spark_time_energy.pdf}
    %\vspace{-0.2cm}
    \caption{\emph{As battery capacity increases, the time and energy to complete a Spark job on volatile solar power decreases due to lower recomputation overhead.}}
    %\vspace{-0.2cm}
%    This graph completes the other one by showing the effect of this on both time and energe. As shown the highr the capacity the less total time and energy it takes.}
    \label{fig:spark_time_energy}
\end{figure}

Figure~\ref{fig:webserver-app}(a) shows the variations over time for both the carbon-intensity and the workload, which are not aligned.  That is, there are periods of both high carbon and workload intensity. Figure~\ref{fig:webserver-app}(b) and (c) shows both the 95$^{th}$\% latency and the rate of carbon emissions over time. A shown in (b), the rate-limiting policy violates the latency SLO near the end of the trace due to a period of both high carbon and workload intensity, since it does not have the flexibility to increase its carbon emissions during this time, as shown in (c). In contrast, the budgeting policy always satisfies the latency SLO even though it has high carbon emissions near the end of the trace.   Note that the rate-limiting policy occasionally provides much better latency than our SLO (by over-provisioning when carbon is low), while the budgeting policy incentivizes our application to not arbitrarily over-provision, but instead pay back some of the carbon it uses to satisfy load spikes. As a result, the budgeting policy always provides service near the SLO.   Overall, the budgeting policy has 27\% lower carbon emissions compared to the rate-limiting policy, since it operates well below the target carbon rate most of the time.   Finally, Figure~\ref{fig:webserver-app}(d) shows how the number of workers varies over the course of the experiment: the budgeting policy uses fewer resources and energy when carbon emissions are low, i.e., only enough to satisfy the SLO, while the rate-limiting policy uses as much resources and energy to satisfy its target carbon rate. 





%the carbon emissions over time for both policies, as well as the request load, while Figure~\ref{fig:server}(bottom) shows the 95$^th$\% latency for both policies.   As shown, rate-limiting carbon results in sudden spikes in the 95$^th$\% latency when both carbon emissions and load are high.  In contrast, budgeting carbon is capable of maintaining a steady 95\% latency by reducing resource and energy usage when load is low (under both high and low carbon emissions). Note that when rate-limiting carbon, our application occasionally provides much higher latency than our SLO (by over-provisioning when carbon is low), while carbon budgeting incentivizes our application to not arbitrarily over-provision, but instead pay back some of the carbon it uses to satisfy load spikes.





\subsection{Leveraging Batteries}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.4\textwidth]{figures/spark/spark_workers_change.pdf}
% \includegraphics[width=0.4\textwidth]{figures/spark/spark_time_energy.pdf}
% \vspace{-0.5cm}
% \caption{\emph{Number of active workers (right y-axis) for a Spark application running on solar power (left y-axis) over time (x-axis) using different battery capacities (top).  Total running time (left y-axis) and solar energy usage (right y-axis) as a function of battery capacity (x-axis) for the same application.}}
% \vspace{-0.5cm}
% \label{fig:spark}
% \end{figure}

The applications above focus on optimizing carbon-efficiency using grid power that has a variable carbon intensity.  Of course, many applications have temporal flexibility, and can thus run directly on solar power, which is infinitely carbon-efficient.  However, the disadvantage of running directly on solar power is its volatility due to changing environmental conditions. While applications can often handle this volatility, e.g., using fault-tolerance mechanisms, they can incur additional performance and energy overheads.  To illustrate, we ran a distributed Spark application without modification on our ecovisor prototype that is powered by intermittent solar.  In this case, the application is an image preprocessing and feature extraction job written using pyspark and run on Spark 3.2.0. The application horizontally scales its number of workers (and its aggregate power usage) to match the solar power, and does not perform periodic checkpointing.  Thus, when solar power decreases, workers are terminated and lose any data stored in volatile memory.  While Spark is resilient to these terminations and automatically recomputes any lost data, the recomputations increase the application's total energy usage and running time.  Thus, while running on volatile solar (or wind) energy is infinitely carbon-efficient, these overheads can make it highly energy-inefficient.  We also show the pseduo-code for our battery-aware Spark auto-scaling policy using our ecovisor API in Algorithm \ref{alg.battery}. 

Here, we can use our ecovisor to mitigate solar's volatility and corresponding overhead using energy storage. Algorithm \ref{alg.battery} shows the scaling policy under intermittent solar power availability that uses batteries to mitigate volatility. The algorithm takes $min\_power$ as an input that is configured based on an application's needs and battery charge. To manage solar volatility, there are two cases. In the first case, in any interval where there is excess solar power, we use the excess to charge the battery and we increase the number of containers by one. In the second case, where there is no excess solar power, if the available solar power is less than the minimum power, we discharge the battery to provide the minimum power $min\_power$.  We then scale the number of containers up or down to match the available power. 

%\vspace{-0.3cm}
\begin{algorithm}[t]
{\scriptsize
\caption{Battery-aware Spark Auto-Scaler Policy}
\label{alg.battery}
\begin{algorithmic}[1]
\REQUIRE \ $min\_power$\\
\FOR{each t$=1,2, \dots$}
\STATE ${app\_power = {\fontfamily{qcr}\selectfont get\_app\_power()}}$
\STATE ${solar\_power = {\fontfamily{qcr}\selectfont get\_solar\_power()}}$
\STATE ${delta\_power = solar\_power - app\_power}$
\IF {$delta\_power > 0$}
\STATE ${\fontfamily{qcr}\selectfont set\_battery\_charge\_rate(delta\_power-  {\fontfamily{qcr}\selectfont get\_container\_power())})}$
\STATE ${containers(t) = containers(t-1)+1}$
\ELSE
    % \STATE ${\fontfamily{qcr}\selectfont set\_battery\_power(min\_power)}$
    \STATE ${\fontfamily{qcr}\selectfont available\_power = max(min\_power, solar\_power)}$
    %\STATE ${containers(t) = int(available\_power/}$
    %\STATE $ \quad \quad \quad \quad \quad \quad \quad \quad  {\fontfamily{qcr} \selectfont get\_container\_power())}$\\
    \STATE ${containers(t) = \Bigl \lfloor \dfrac{available\_power}{get\_container\_power()}\Bigr\rfloor}$
    %\STATE $ \quad \quad \quad \quad \quad \quad \quad \quad  {\fontfamily{qcr} \selectfont get\_container\_power())}$\\
\ENDIF
\ENDFOR
\end{algorithmic}
}
\end{algorithm}
%\vspace{-0.4cm}

Figure~\ref{fig:spark} shows the results.  Figure~\ref{fig:spark}(top) shows a time-series that includes the solar generation (a) and number of Spark workers with (c) and without (b) a battery.  In this case, the battery has a capacity of 600Wh.   Our application controls the battery to provide backup power when solar power drops, which reduces the number of workers terminated and the recomputation overhead.   As shown, the Spark job completes substantially earlier, and uses less energy, when using the battery to mitigate solar volatility due to the lower recomputation overhead. Figure~\ref{fig:spark_time_energy} shows that as the battery capacity increases both the time and energy required to complete the job decreases due to the lower recomputation overhead. This experiment demonstrates that enabling applications to control energy storage provides a useful mechanism for reducing clean energy volatility, and its associated overhead. 
 
 
%   Figure~\ref{fig:spark}(bottom) shows that as the battery capacity increases both the total running time and energy consumed also decreases. This experiment demonstrates that control of energy storage provides a useful mechanism for reducing renewable energy's volatility, and its associated overhead. 

% \begin{figure*}[t]
%     \centering
%     \begin{tabular}{ccc}
%     \includegraphics[width=0.3\textwidth]{./figures/balancing_application/balancing_illustrative.pdf}
%     &
%     \includegraphics[width=0.3\textwidth]{./figures/balancing_application/container_power.pdf}
%     &
%     \includegraphics[width=0.3\textwidth]{./figures/balancing_application/balancing_result.pdf}\\
%     (a) Solar power & 
%     (b) Per-container power caps  &
%     (c) Runtime and Energy-efficiency \\
%     \end{tabular}
%     %\vspace{-0.2cm}
%     \caption{\emph{Comparison of a dynamic and static policy for setting per-container power caps (b) for a parallel job running across 10 nodes using the solar energy in (a). The dynamic policy's improvement in runtime and energy-efficiency is shown in (a).}}
%     %\vspace{-0.3cm}
%     \label{fig:balancing-app}
% \end{figure*}

\begin{figure}[t]
    \centering
    \begin{tabular}{c}
    \includegraphics[width=\columnwidth]{figures/balancing_application/balancing_illustrative.pdf}\\
    (a) Solar power\\
    \includegraphics[width=\columnwidth]{figures/balancing_application/container_power.pdf}\\
    (b) Per-container power caps\\
    \includegraphics[width=\columnwidth]{figures/balancing_application/balancing_result.pdf}\\
    (c) Runtime and Energy-efficiency\\
    \end{tabular}
    %\vspace{-0.2cm}
    \caption{\emph{Comparison of a dynamic and static policy for setting per-container power caps (b) for a parallel job running across 10 nodes using the solar energy in (a). The dynamic policy's improvement in runtime and energy-efficiency is shown in (a).}}
    %\vspace{-0.2cm}
    \label{fig:balancing-app}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \begin{tabular}{c}
%     \includegraphics[width=0.4\textwidth]{./figures/balancing_application/balancing_illustrative.pdf}\\
%     (a) Solar power\\
%     \includegraphics[width=0.4\textwidth]{./figures/balancing_application/container_power.pdf}\\
%     (b) Per-container power caps\\
%     \includegraphics[width=0.4\textwidth]{./figures/balancing_application/balancing_result.pdf}\\
%     (c) Runtime and Energy-efficiency\\
%     \end{tabular}
%     \vspace{-0.1cm}
%     \caption{\emph{Comparison of a dynamic and static policy for setting per-container power caps (b) for a parallel job running across 10 nodes using the solar energy in (a). The dynamic policy's improvement in runtime and energy-efficiency is shown in (a).}}
%     \vspace{-0.2cm}
%     \label{fig:balancing-app}
% \end{figure}


\subsection{Directly Exploiting Solar Power}

Some parallel applications may be able to more directly exploit solar power with little battery capacity, despite its volatility, using vertical scaling.   Since our ecovisor enables applications to balance power's supply and demand themselves, these applications can explicitly allocate their limited solar power across their set of containers, e.g., such that the sum of containers' power caps does not exceed the supply of solar power.  In this case, applications should allocate their limited solar power to where it can be used most productively.  Since servers are not energy-proportional, they consume some power even when idle.  Thus, servers' most energy-efficient operating point is at 100\% of their allocated energy, and any idleness due to operating below this point wastes some energy.    However, parallel applications often have tasks that are idle due to performing I/O, as with our Spark job above, or from periodically synchronizing across tasks, as with training EfficientDet-d1 above.  These types of parallel applications often exhibit stragglers tasks that can increase running time by forcing other tasks to wait~\cite{straggler1,straggler2,straggler3}. 

Importantly, executing parallel applications on a limited amount of solar power can exacerbate the performance issues above.  To illustrate, Figure~\ref{fig:balancing-app}(a) shows solar power over a day, along with a parallel job, which periodically synchronizes across tasks and performs I/O, using vertical scaling across 10 nodes to match the available solar power. In this case, we implement two power capping policies: one that sets static caps across all 10 nodes, and another that sets caps to ensure each node uses near 100\% of its allocated energy, i.e., uses near 100\% utilization of its allocated resources.  Figure~\ref{fig:balancing-app}(b) shows how the dynamic power caps differ across the 10 nodes relative to the static cap (center line) over the trace.  Figure~\ref{fig:balancing-app}(c) scales the solar output from (a) by the percentage on the x-axis and plots the runtime improvement from using the dynamic policy (left y-axis) and its energy-efficiency (right y-axis).  The graph shows that as solar energy decreases, the importance of dynamically balancing power to reduce runtime increases.  Energy-efficiency increases as available solar power increases, since each node's base power is amortized over more productive work, which again illustrates the inefficiency of solar power. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/straggler_application/results.pdf}
    %\vspace{-0.1cm}
    \caption{\emph{Mitigating stragglers using replica tasks is one way to productively consume excess renewable energy.}}
    \label{fig:straggler-app}
    %\vspace{-0.2cm}
\end{figure} 

Finally, Figure~\ref{fig:straggler-app} shows the same application as we scale the solar output from Figure~\ref{fig:balancing-app}(a) up, which results in an excess of solar energy.   If applications cannot store the excess energy, they are incentivized to use it immediately, even if that usage is not entirely efficient.  To illustrate, we configure our parallel job to perform straggler mitigation by tracking the progress of each task and issuing a replica for any slow tasks~\cite{straggler1,straggler2,straggler3}.   For this experiment, we randomly inject straggler tasks to highlight our point.  Figure~\ref{fig:straggler-app} shows that as solar energy increases, our application's overall energy-efficiency decreases, since we consume that energy by spawning more task replicas.   However, this absolute decrease in energy-efficiency is not important, since the excess solar energy would have been otherwise wasted. In this case, we improve the runtime by using the excess energy for straggler mitigation, although we see diminishing returns as we submit more replicas (since at most one replica task will finish).  

%The scenarios above focus on regulating carbon emissions from using grid power.  Of course, applications that have access to onsite renewable energy sources can eliminate their carbon emissions by solely using renewable energy. 

%We have a parallel  HPC application that operates under a variable power supply (due to renewable energy or variable carbon).  The application must allocate its power correctly to optimize performance using vertical scaling.  The parallel application must have some imbalance for this to work; that is, nodes operate at different changing utilizations, which requires some dynamic re-balancing of power.  We show one case with static power, and unchanging power caps.  We show another case with re-balancing, and the re-balancing case should perform better (finish faster).  We could also do this experiment with the distributed web server and show latency instead of finishing time.   
%
%%Utilizing Excess Renewables (straggler mitigation)
%
%We have some parallel application that implements straggler mitigation (e.g., spawning replica tasks to reduce the impact of stragglers).   When renewable energy is high (and if it cannot be stored) then we spawn more stragglers to reduce the running time by some amount.  Since we cannot store the energy, using it for stragglers is useful even if more stragglers is not entirely efficient, i.e., much of their computation is wasted. 

%The application is Spark executing some job.  We run the job using reliable grid power, and it finishes in some time using some amount of energy.  Importantly, the job dictates when it needs energy and the grid supplies it.  We run on the job using only variable solar energy.  When solar energy drops, we have to kill some containers, which in Spark results in the loss of volatile memory state.  Spark automatically re-computes this lost state.  Thus, when using variable solar energy, the job will take longer and consume more total energy when using the grid.  Solar energy is not energy-efficient due to the variations. We then show how we can use our virtual battery to make the solar energy look more like the grid energy, and have a completion time and energy use closer to the grid.  We show that the battery energy losses ($\sim$5\%) are less than the energy losses from using solar energy (more than 5\%).  The point is that applications can use their virtual energy system and battery to improve performance.



%Our evaluation illustrates the flexibility of our ecovisor to support multiple types of carbon-aware applications with different performance requirements, including distributed ML training, elastic and inelastic HPC applications, e.g., using MPI, a distributed web application, and bulk-synchronous data-parallel jobs, e.g., via Spark.  As we discuss, some of these carbon-aware applications have been the subject of prior work.   Importantly, our approach supports these existing applications, as well as provides a platform for i) developing new carbon-aware application and abstractions and ii) running many different applications concurrently on the same shared infrastructure.  We examine each application under a different energy mix and constraints that affect how it uses its virtual energy system to optimize carbon-efficiency and performance. In doing so, our evaluation highlights key elements of carbon-efficient design that have not been well-studied. 


%We first demonstrate how our ecovisor enables applications that are responsive to varying carbon-intensity of grid energy.  
%
%In this case, our application is distributed ML training of a XX model for XX using pytorch that runs on 8 GPUs, and runs solely on grid power.   The application uses ecovisor's functions for monitoring grid energy's carbon-intensity and power usage, and can use both horizontal and vertical scaling to regulate its power usage, e.g., by starting/stopping containers and setting per-container power caps.   We then implement a simple carbon-aware policy from recent work, called WaitAWhile~\cite{wait-awhile}, that reduces carbon emissions by stopping the application whenever grid energy's carbon-intensity exceeds some pre-defined upper threshold.  We also implemented our own simple variant of this policy, called Wait\&Scale, which also horizontally scales up (by a fixed amount XX) the number of containers used, and thus power usage, when grid energy's carbon-intensity drops below some lower threshold.   We compare these policies to a carbon-agnostic policy that simply runs the job as normal to completion on the fixed-size cluster.
%
%We ran the distributed ML training job above for each policy assuming a carbon-intensity trace from California, e.g., CALISO, in 20XX.   Since California has a high renewable penetration, its grid carbon-intensity exhibits significant daily variations.  Since the extent of these daily variations are weather-dependent, we ran the experiment 10 times with different randomly chosen starting times.  In addition, we also scaled down both our job size and running time, as well as our carbon trace, by 60$\times$ to enable more rapid experimentation, i.e., each minute of our experiment would correspond to one hour in practice.   Carbon-intensity changes on hourly time-scales, so running numerous experiments in real time and large scales is impractical. Figure~\ref{fig:carbon-responsive} shows the results, where the left y-axis is average carbon emissions, the right y-axis is average completion time, the x-axis represents the three different policies, and the error bars represent XX across the 10 experiments. As expected, the carbon-agnostic policy finishes in least time, but has the highest carbon emissions, while the WaitAWhile policy has lower carbon emissions (by 24.4\%) but has a significantly longer completion time.  In addition, the WaitAWhile policy has high variance in its completion time, since it is entirely dependent on the carbon-intensity: if it remains high for a long period, it makes no forward progress.  By contrast, our simple Wait\&Scale policy slightly increases the carbon emissions compared to WaitAWhile, but significantly decreases both the average completion time (by nearly 4$\times$) and its variance. 
%
%Our results above motivate further research in developing carbon-responsive applications, which our ecovisor can enable.  Our Wait\&Scale policy is basic, as it scales up a fixed amount if carbon-intensity drops below a pre-defined threshold.  Determining the optimal scaling is more complex for distributed applications, as scaling up increases both communication costs and can cause synchronization delays, which affects carbon-efficiency by decreasing energy-efficiency. As a result, scaling up too much, even when grid carbon-intensity is low, can increase overall carbon emissions.  Figure~\ref{fig:carbon-scaling} illustrates this point by varying the number of GPUs used to train the model above on the x-axis, and plotting the carbon-efficiency, i.e., work done (1 job) per total carbon emissions, on the left y-axis and and completion time on the right y-axis.   The completion time increases non-linearly due to communication and synchronization costs, which causes the carbon-efficiency to decrease as the application scales up. 

%We have an elastic parallel application (distributed ML training) that periodically communicates to synchronize. When carbon is low, the application can scale up to use more energy.  However, its carbon-efficiency decreases the more it scales up due to communication overhead.  We scale up to the knee of the curve, which is the most carbon-efficient point. When carbon is high, we scale down.  We just have some simple thresholds.  We compare with an inelastic version of the application. 

%ML training using pytorch cluster. 8 GPUs and 8 nodes on AWS. Use three traces of carbon. Deep learning training for object detection; coco dataset. Naive - just run everything. Stop policies: stop if carbon efficiency is higher than threshold. Different number of GPUs; 0-15. 


%s: a carbon-agnostic static policy that never varies the number of resources, a carbon rate-limiting policy that uses horizontal scaling to limit carbon emissions, and a carbon rate-limiting policy that uses both horizontal and vertical scaling to limit carbon emissions. 
%policy and a policy that rate-limits its carbon emissions to XX g$\cdot$CO$_2$/s.  
%We implement two rate-limiting policies: one that only uses horizontal scaling to adjust carbon emissions, and one that uses both horizontal and vertical scaling.  
%shows a time-series of running BLAST
%and aga
%, while rate-limiting carbon over a representative day using the CAISO carbon trace. 
%In this case 
%finds regions of similarity between biological sequences. The program compares nucleotide or protein sequences to sequence databases and calculates the statistical significance.

%Another approach to regulating carbon is to simply rate-limit it by capping an application's carbon emissions at a fixed level over time.    %Given a carbon cap, grid power's variable carbon-intensity dictates a variable amount of grid power that is available to applications.   

% Our ecovisor can enable both platforms to enforce carbon caps and applications to respond to them. Carbon caps incentivize applications to use the energy that is available to them (even if they use it inefficiently), and are thus simpler than the carbon-responsive applications above, which require determining complex trade-offs between carbon-efficiency and performance.   Of course, as with the applications above, carbon caps are most appropriate for non-interactive batch applications that can tolerate some delay in their completion time, since long periods of high carbon-intensity may limit energy availability.  
%
%Figure~\ref{fig:hpc} shows results for a distributed elastic HPC application, which does XXX, that is subjected to a carbon cap.  In this case, the HPC application only uses grid power, and horizontally scales the number of containers to regulate its power usage as grid power's carbon-intensity, and its power availability, vary over time.  In this experiment, we use the same trace of grid carbon-intensity as above from CALISO over 20XX.  The x-axis is XX and the y-axis is XX. Need more here XXX. 

%The application is a distributed web server executing web requests with some latency.  A carbon cap dictates a fixed rate of carbon emissions at all times.  Thus, a fixed carbon cap requires the application to varies its energy usage as carbon intensity varies.  As a result, if carbon intensity is high, then the application has to use less energy, even if its demand is high. A carbon budget that provides applications the flexibility to "spend" carbon over a longer period of time, e.g., week or month, gives applications the freedom to choose when to use carbon.  We subject our web server to variable application demand and record its latency under a carbon cap.  The latency will be especially bad when carbon is high and demand is high (due to fewer resources).  We then show an application with a carbon budget that equals the cap.  In this case, we vary our carbon usage according to demand to maintain latency below some threshold.  We set the threshold so the experiment works out correctly.  We use more carbon when demand is high to satisfy the latency target, even if the carbon is high. 



